Pond: CXL-Based Memory Pooling Systems for Cloud Platforms

Public cloud providers seek to meet stringent performance requirements and low hardware cost. A key driver of performance and cost is main memory. Memory pooling promises to improve DRAM utilization and thereby reduce costs. However, pooling is challenging under cloud performance requirements. This paper proposes Pond, the first memory pooling system that both meets cloud performance goals and significantly reduces DRAM cost. Pond builds on the Compute Express Link (CXL) standard for load/store access to pool memory and two key insights. First, our analysis of cloud production traces shows that pooling across 8-16 sockets is enough to achieve most of the benefits. This enables a small-pool design with low access latency. Second, it is possible to create machine learning models that can accurately predict how much local and pool memory to allocate to a virtual machine (VM) to resemble same-NUMA-node memory performance. Our evaluation with 158 workloads shows that Pond reduces DRAM costs by 7% with performance within 1-5% of same-NUMA-node VM allocations.

==> Makefile <==
#-------------------------------------------------------------------------------
#
# Makefile to compile the paper
# Usage:
#     - ``make h``: compile the tex files into "main.pdf"
#     - ``make p``: compile and open "main.pdf" using ~/bin/pdfreader (wrapper
#       of evince, mpdf, zathura, etc.)
#
#-------------------------------------------------------------------------------

MAIN      = main
SRCS      = *.tex
PS        = $(MAIN).ps
PDF       = $(MAIN).pdf
DVI       = $(MAIN).dvi
TARG      = $(MAIN).done

all: texnoredo cleanabit

h: all cleanabit # ps pdf

p: all openpdf cleanabit #ps pdf

s: openpdf

b: main.pdf
	${HOME}/bin/backup-file main.pdf

openpdf:
	${HOME}/bin/pdfreader main.pdf

diff:
	docs/diff.sh 44851a377ff7398da9ba5bdcea1d47facee077ee

texwithredo:
	pdflatex main.tex
	bibtex -min-crossrefs=1000 main
	pdflatex main.tex
	pdflatex main.tex

texnoredo:
	pdflatex main.tex
	bibtex -min-crossrefs=1000 main
	pdflatex main.tex
	pdflatex main.tex

e:
	pdflatex extended_abstract.tex
	bibtex -min-crossrefs=100 extended_abstract
	pdflatex extended_abstract.tex
	pdflatex extended_abstract.tex

texnobib:
	pdflatex main.tex

$(MAIN).bbl: $(MAIN).aux
	bibtex -min-crossrefs=200 $(MAIN)
	./redo-bib.csh $(MAIN)

$(MAIN).aux: $(MAIN).tex
	latex $(MAIN)

ps: $(DVI)
	dvips -o $(PS) $(MAIN)

pdf: $(PS)
	ps2pdf14 $(PS)

clean:
	rm -vf *.ps  main.pdf *.dvi *.aux *.log \
	*.bbl *.blg *.out *.brf *.4*  \
	*.css *.idv *.lg *.tmp *.xref *.png *.toc

cleanabit:
	rm -vf *~ *.ps  *.aux *.log \
	*.bbl *.blg *.out *.brf *.4*  \
	*.css *.idv *.lg *.tmp *.xref *.png *.toc


==> asplos.tex <==

% TO FIX (taken from ASPLOS'20 for LeapIO)

\copyrightyear{2023}
\acmYear{2023}
\setcopyright{acmlicensed}
\acmConference[ASPLOS '23]{Proceedings of the Twenty-Eighth International Conference on Architectural Support for Programming Languages and Operating Systems}{March 16--20, 2023}{Vancouver, Canada}
\acmBooktitle{Proceedings of the Twenty-Eighth International Conference on Architectural Support for Programming Languages and Operating Systems (ASPLOS '23), March 16--20, 2023, Vancouver, Canada}
\acmPrice{15.00}
\acmDOI{10.1145/3373376.3378531}
\acmISBN{978-1-4503-7102-5/20/03}

%\fancyhead{}

%=======================================================================
% ACM specific
%=======================================================================
%\pgfplotsset{compat=1.17}
\widowpenalty=0
\clubpenalty=0
\brokenpenalty=0


==> cite-p-mem.tex <==

\subsection{Memory Disaggregation Bibs}

\cite{flash.isca94} :: The Stanford FLASH multiprocessor \\
\cite{javatps.ispass13} :: Increasing the Transparent Page Sharing in Java \\
\cite{javastringdedup.vee14} :: String Deduplication for Java-based Middleware in Virtualized Environments \\
\cite{disaggmemperfmodel.memsys20} :: Performance Modeling and Evaluation of a Production Disaggregated Memory System \\
\cite{dissmemruntime.asplos21} :: Rethinking Software Runtimes for Disaggregated Memory \\
\cite{aifm.osdi20} :: AIFM: High-Performance, Application-Integrated Far Memory \\
\cite{semeru.osdi20} :: Semeru: A Memory-Disaggregated Managed Runtime \\
\cite{resdisagg.osdi16} :: Network Requirements for Resource Disaggregation \\
%\cite{sparkdisagg.ancs16} :: Is Memory Disaggregation Feasible? A Case Study with Spark SQL \\
%\cite{orchdisaggmem.tc20} :: Hierarchical Orchestration of Disaggregated Memory \\
\cite{dspm.socc17} :: Distributed Shared Persistent Memory \\
\cite{zombieland.eurosys18} :: Welcome to zombieland: Practical and Energy-efficient memory disaggregation in a datacenter \\
\cite{thymesisflow.micro20} :: ThymesisFlow: A Software-Defined, HW/SW Co-Designed Interconnect Stack for Rack-Scale Memory Disaggregation \\
\cite{pberry.hotos19} :: Project PBerry: FPG Aacceleration for Remote Memory \\
\cite{fastnetdisagg.socc17} :: Remote Memory in the Age of Fast Networks \\
\cite{dredbox.date16} :: Rack-scale Disaggregated Cloud Data Centers: The dReDBox project vision \\
\cite{memblade.isca09} :: Disaggregated Memory for Expansion and Sharing in Blade Servers \\
\cite{sysdisaggmem.hpca12} :: System-level Implications of Disaggregated Memory \\
%\cite{dcm.tc19} :: Disaggregated Cloud Memory with Elastic Block Management \\
\cite{transrm.web19} :: Enabling Efficient and Transparent Remote Memory Access in Disaggregated Datacenters \\
\cite{memdisaggrsch.icdcs19} :: Memory Disaggregation: Research Problems and Opportunities \\
\cite{infiniswap.nsdi17} :: Efficient Memory Disaggregation with INFINISWAP \\
\cite{softfarmem.asplos19} :: Software-Defined Far Memory in Warehouse-Scale Computers \\
\cite{vmembigserver.isca13} :: Efficient Virtual Memory for Big Memory Servers \\
\cite{rmemmap.isca15} :: Redundant Memory Mappings for Fast Access to Large Memories \\
\cite{prefetchats.micro19} :: Prefetched Address Translation \\
\cite{learnedpagetableindex.nips18} :: Virtual Address Translation via Learned Page Table Indexes \\
\cite{legoos.osdi18} :: LegoOS: A Disseminated, Distributed OS for Hardware Resource Disaggregation \\
%\cite{rackmemdisagg.samos17} :: A Software-defined Architecture and Prototype for Disaggregated Memory Rack Scale Systems \\
\cite{ememdisagg.web19} :: Mitigating the Performance-Efficiency Tradeoff in Resilient Memory Disaggregation \\
\cite{fastswap.eurosys20} :: Can Far Memory Improve Job Throughput? \\
\cite{fluidmem.icdcs20} :: FluidMem: Full, Flexible, and Fast Memory Disaggregation for the Cloud \\
%\cite{disaggmemperf.cf20} :: Contention-aware Application Performance Prediction for Disaggregated Memory Systems \\
\cite{hwdemandpaging.isca20} :: A Case for Hardware-Based Demand Paging \\
\cite{dbmsdisagg1.cidr20} :: Rethinking Data Management Systems for Disaggregated Data Centers \\
\cite{dbmsdisagg2.vldb20} :: Understanding the Effect of Data Center Resource Disaggregation on Production DBMSs \\
\cite{kvdisagg.atc20} :: Disaggregating Persistent Memory and Controlling Them Remotely: An Exploration of Passive Disaggregated Key-Value Stores \\
\cite{leap.atc20} :: Effectively Prefetching Remote Memory with Leap \\
\cite{vmitosis.asplos21} :: Fast Local Page-Tables for Virtualized NUMA Servers with vMitosis \\
\cite{mitosis.asplos20} :: Mitosis: Transparently Self-Replicating Page-Tables for Large-Memory Machines \\
%\cite{adaptpagemigration.tc20} :: Adaptive Page Migration Policy with Huge Pages in Tiered Memory Systems \\
\cite{uksm.fast18} :: UKSM: Swift Memory Deduplication via Hierarchical and Adaptive Memory Region Distilling \\
\cite{akc.socc17} :: AKC: Advanced KSM for cloud computing \\
\cite{specjvm08.web} :: SPECjvm 2008 \\
\cite{dacapo.web} :: DaCapo Benchmarks \\
\cite{renaissance.web} :: Renaissance Suite \\
%\cite{dlbench.cloud20} :: The Design and Implementation of a Scalable Deep Learning Benchmarking Platform \\
\cite{ldbcbench.web} :: The LDBC Graphalytics Benchmark \\
%\cite{syncdeeprl.neurips2020} :: High-Throughput Synchronous Deep RL \\
%\cite{memaccel.arxiv2020} :: Accelerating Bandwidth-Bound Deep LearningInference with Main-Memory Accelerators \\
\cite{hawkeye.asplos19} :: HawkEye: Efficient Fine-grained OS Support for Huge Pages \\
\cite{nimblepage.asplos19} :: Nimble Page Management for Tiered Memory Systems \\
\cite{thermostat.asplos17} :: Thermostat: Application-transparent Page Management for Two-tiered Main Memory \\
%\cite{specpaging.memsys17} :: Speculative Paging for Future NVM Storage \\
\cite{heteroos.isca17} :: HeteroOS: OS Design for Heterogeneous Memory Management in Datacenters \\
%\cite{kloc.arxiv20} :: Efficient Kernel Object Management for Tiered Memory Systems with KLOC \\
\cite{netdimm.micro19} :: NetDIMM: Low-Latency Near-Memory Network Interface Architecture \\
\cite{datatiering.eurosys16} :: Data Tiering in Heterogeneous Memory Systems \\
\cite{hybridmem.ics11} :: Page Placement in Hybrid Memory Systems \\
%\cite{..arxiv20} :: Hardware Memory Management for Future Mobile Hybrid Memory Systems \\
\cite{flatflash.asplos19} :: FlatFlash: Exploiting the Byte-Accessibility of SSDs within a Unified Memory-Storage Hierarchy \\
\cite{scalepm.fast20} :: An Empirical Guide to the Behavior and Use of Scalable Persistent Memory \\
\cite{optaneeval.memsys19} :: System Evaluation of the Intel Optane Byte-addressable NVM \\
%\cite{optanedbms.damon20} :: Lessons Learned from the Early Performance Evaluation of Intel Optane DC Persistent Memory in DBMS \\
\cite{hybridtiering.ismm20} :: Exploiting Inter- and Intra-Memory Asymmetries for Data Mapping in Hybrid Tiered-Memories \\
\cite{hinuma.iccd19} :: HiNUMA: NUMA-Aware Data Placement and Migration in Hybrid Memory Systems \\


==> fig-contactcount.tex <==
\begin{figure}[t!]
  \centering
\includegraphics[width=0.8\columnwidth]{F/sketches/contact_count}
\mycaption{fig-contactcount}{External memory controller (EMC) overview}{The EMC ASIC can connect multiple DDR5 DIMMs and CXL hosts. For example, four DDR5 DIMMS and 16 \tms{8}-CXL links would require about 3000 contacts, less than a 2016-gen LGA-3647 socket~\cite{intel2019xeon}.}
\end{figure}


==> fig-cxl-cdf.tex <==


\def \hmina {\hspace{0.0in}}
\def \hminb {\hspace{-0.35in}}

\def \fgw {1.2in}
\def \fgh {1.085in}


\begin{figure}[t!]
\centerline{
\hmina
\includegraphics[width=\fgw]{F/cxl/eps/cxl-slowdown-cdf.pdf}
\hminb
\includegraphics[width=\fgw]{F/cxl/eps/membw-cdf.pdf}
\hminb
\includegraphics[width=\fgw]{F/cxl/eps/wss-cdf.pdf}
\hminb
\includegraphics[width=\fgw]{F/cxl/eps/cpi-slowdown-cdf.pdf}
}

\vminfive

\mycaption{fig-cxl-cdf}{CXL slowdowns and metrics}{CDFs of CXL
    performance slowdown, workload DRAM bandwidth and working set size
    of all the \numTotalApps\ workloads}{}

\vminten

\end{figure}


==> fig-discussion-scope.tex <==

\def \vmina {\vspace{-0.1in}}
\def \vminb {\vspace{0.05in}}

\begin{figure}[t!]
\centering
\includegraphics[width=0.25\columnwidth]{F/sketches/discussion-scope}
\vmina
\caption{CXL connection proposal to shift capacity between pools larger than eight sockets.}
\label{fig-discussion-scope}

\vminb

\end{figure}




==> fig-interleave-cdf.tex <==

\def \hmina {\hspace{-0.1in}}
\def \hminb {\hspace{-0.2in}}

\def \fgw {2.0in}
\def \fgh {1.085in}

% \begin{floatingfigure}[r]{2in}  (and \end{..})

\begin{figure}[t!]

\centerline{
% \hmina
\includegraphics[width=\fgw]{F/cxl/eps/interleave-cdf.pdf}
}
%
\vminten
%
\mycaption{fig-interleave-cdf}{Workload performance slowdown under
interleaving memory policy}{}
%
\vminten

\end{figure}



==> fig-interleave.tex <==

\def \hmina {\hspace{-0.1in}}
\def \hminb {\hspace{-0.2in}}

\def \fgw {7.2in}
\def \fgh {1.085in}

% \begin{floatingfigure}[r]{2in}  (and \end{..})

\begin{figure*}[t!]

\centerline{
% \hmina
\includegraphics[width=\fgw]{F/interleave/eps/all.pdf}
}

\begin{comment}
% \hmina \includegraphics[width=\fgw]{F/empty.eps} \hminb
\includegraphics[width=\fgw]{F/interleave/eps/cpu2017.pdf} } \vminten
\centerline{ \includegraphics[width=\fgw]{F/interleave/eps/gapbs.pdf} }
\end{comment}
%
\vminten
%
\mycaption{fig-interleave}{Performance slowdown under interleaving
memory allocation policy for SPEC CPU 2017 and GAPBS. ``Local-First''
denotes the default memory policy \sys uses, and ``Interleaving'' policy
performs page-level striping across local and CXL memory}{}
%
\vmintwenty

\end{figure*}



==> fig-kv.tex <==

\def \hmina {\hspace{-0.1in}}
\def \hminb {\hspace{-0.1in}}

\def \fgw {1.78in}
\def \fgh {1.085in}

% \begin{floatingfigure}[r]{2in}  (and \end{..})

\begin{figure}[t!]
\centerline{
\hmina
\includegraphics[width=\fgw]{F/kv/eps/voltdb-a-thru-vs-rd-lat.pdf}
\hminb
\includegraphics[width=\fgw]{F/kv/eps/voltdb-a-thru-vs-rd-lat.pdf}
}

\vminten

\mycaption{fig-kvlat}{VoltDB Throughput vs. Latency}{YCSB-A read latency
(Y-axis) under various throughput targets (X-axis).}

\vminfifteen

\end{figure}



==> fig-kvlat.tex <==
\def \hmina {\hspace{-0.1in}}
\def \hminb {\hspace{-0.1in}}

\def \fgw {1.78in}
\def \fgh {1.085in}

% \begin{floatingfigure}[r]{2in}  (and \end{..})

\begin{figure}[t!]
\centerline{
\hmina
\includegraphics[width=\fgw]{F/kv/eps/voltdb-a-thru-vs-rd-lat.pdf}
\hminb
\includegraphics[width=\fgw]{F/kv/eps/voltdb-a-thru-vs-rd-lat.pdf}
}

\vminten

\mycaption{fig-kvlat}{VoltDB Throughput vs. Latency}{YCSB-A read latency
(Y-axis) under various throughput targets (X-axis).}

\vminfifteen

\end{figure}



==> fig-memoryutil.tex <==

\def \hmina {\hspace{-0.1in}}
\def \hminb {\hspace{-0.2in}}

\begin{figure}[t!]
\hmina
\centering
\includegraphics[width=0.8\columnwidth]{F/stranding/memory_util}
\vspace{-.1in}
\mycaption{fig-memoryutil}{Memory utilization in VMs observed at \azure. Most VMs use only a fraction of their allocated DRAM}{}

\vminten
\vspace{-.1in}
\end{figure}




==> fig-memutil.tex <==

\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.95\columnwidth]{F/stranding/memory_util_cluster}
\mycaption{fig-memoryutil}{Untouched memory at \azure}{VMs have a significant amount of untouched
memory.}
\vminten
\end{center}
\end{figure}


==> fig-perfml.tex <==

\begin{figure}[t!]
\includegraphics[width=0.49\columnwidth]{F/stranding/emon_model_small}
\mycaption{fig-ml-sensitivity}{Comparison of three prediction models for whether a workload exceeds its performance target (either 5\% or 10\% degradation)}{}
\end{figure}


\begin{figure}[t!]
\includegraphics[width=0.99\columnwidth]{F/stranding/footprint_model}
\mycaption{fig-ml-frigid}{Comparison of static and ML-based allocation of pool memory. The ML model predicts the amount of untouched memory based on similar VM's behavior in the past}{}
\end{figure}




==> fig-pooling.tex <==

\begin{figure}[t!]
\includegraphics[width=0.99\columnwidth]{F/stranding/pooling_stranding}
\mycaption{fig-pooling}{NOTREALDATA (simulation still running)}{}
\end{figure}




==> fig-split.tex <==

\def \hmina {\hspace{-0.1in}}
\def \hminb {\hspace{-0.15in}}

\def \fgw {7.1in}
\def \fgh {1.085in}

% \begin{floatingfigure}[r]{2in}  (and \end{..})

\begin{figure*}[h!]
%\centerline{
% \hmina
% \includegraphics[width=\fgw]{F/empty.eps}
% \hminb
%\includegraphics[width=\fgw]{F/split/eps/cpu2017.pdf}
%}
%\vminfive
\centerline{
\hmina
%\includegraphics[width=1.5in]{F/cxl/eps/split-slowdown-cdf2.pdf}
%\hminb
\includegraphics[width=\fgw]{F/split/eps/gapbs2.pdf}
}

%\vminfifteen
%
\mycaption{fig-split}{GAPBS graph workloads performance slowdown under
different mixed ratio of local and CXL memory (80\%--0\%)}{}
%
\vminfive

\end{figure*}



==> fig-stranding.tex <==
\begin{figure}[t!]
\begin{center}
%\includegraphics[width=\columnwidth]{F/stranding/stranding_bars}
\includegraphics[width=\columnwidth]{F/stranding/stranding_bars_hcl}
\vminfifteen
%\vspace{-4mm}
    \mycaption{fig-stranding-bars}{Memory stranding (\sec\ref{sec-strand})}{Stranding increases significantly as
more CPU cores are scheduled.}
\vspace{-1mm}
\vminten
\end{center}
\end{figure}


%-----------------------------------------------------------------------
% NOT USED
%-----------------------------------------------------------------------
\begin{comment}
\begin{figure*}[t]
\begin{center}

\begin{subfigure}[b]{.4\linewidth}
\includegraphics[width=\columnwidth]{F/stranding/stranding_bars}
\caption{Stranding averages and outliers}
\label{fig-stranding-bars}
\end{subfigure}
%
%\begin{subfigure}[b]{.42\linewidth}
%\includegraphics[width=\columnwidth]{F/stranding/stranding_cpu_correlation.png}
%\caption{Hourly Stranding Snapshots.}
%\label{fig-stranding}
%\end{subfigure}
%
%\begin{subfigure}[b]{.29\linewidth}
%\includegraphics[width=\columnwidth]{F/stranding/stranding_bitmap1.png}
%\caption{TBD}
%\label{fig-stranding-bitmap1}
%\end{subfigure}
%
\hspace*{12pt}
\begin{subfigure}[b]{.4\linewidth}
\includegraphics[width=\columnwidth]{F/stranding/stranding_bitmap2.png}
\caption{Stranding over time}
\label{fig-stranding-bitmap2}
\end{subfigure}
\newline
\hspace*{-20pt}
\begin{subfigure}[b]{.4\linewidth}
\includegraphics[width=\columnwidth]{F/stranding/pooling_static}
\caption{Pooling savings}
\label{fig-stranding-pooling}
\end{subfigure}
\hspace*{12pt}
\begin{subfigure}[b]{.38\linewidth}
\includegraphics[width=\columnwidth]{F/stranding/memory_util_cluster}
\caption{Memory usage}
\label{fig-memoryutil}
\end{subfigure}
%  in VMs observed at \azure. Most VMs use only a fraction of their allocated DRAM
%\vminfive
%
% VM trace analysis from \azure shows that over thousands of daily
% samples
\mycaption{fig-stranding-all}{Memory stranding}{(a) Stranding increases significantly as
more CPU cores are scheduled, the error bars indicate the 5\th\ and
95\th\ percentile (outliers in red); (b) stranding dynamics change
over time and can affect a broad set of servers, (c) small pools of
around 32 sockets are sufficient to significantly reduce overall memory
needs; and (d) VMs have a significant amount of frigid
memory.}

%
\vminten
%
\end{center}
\end{figure*}
\end{comment}


==> fig-systemsketch.tex <==

\def \hmina {\hspace{0.00in}}
\def \hminb {\hspace{-0.2in}}

\begin{figure}[t!]
\hmina
%\begin{minipage}[t]{0.85\columnwidth}
\centering
\includegraphics[width=0.9\columnwidth]{F/sketches/system_sketch}
%\end{minipage}
%\hspace{0mm}
%\begin{minipage}[t]{0.22\columnwidth}
%\vspace{-26mm}
%\small
%\setlength{\tabcolsep}{1.5pt}
%\begin{tabular}{l|r}
% & Latency\\
%\hline
%CXL phy/ctr & 40ns \\
%Retimer\footnote{\mbox{For large pools}} & 20ns \\
%Propagation & 7ns \\
%EMC & 20ns\\
%\end{tabular}
%\end{minipage}
%\vspace*{-3pt}

% reconfigures the system and enforced security and robustness
\mycaption{fig-systemsketch}{\sys hardware design}{In \sys, each CPU
connects to several external memory controllers (EMC).
Each EMC offers CXL ports for several sockets and DDR ports for
several DIMMs, which constitute the pool. Dashed lines around each CPU and EMC
indicate separate failure domains.
%
}

\vminten

\end{figure}




==> fig-tmam.tex <==

\def \hmina {\hspace{-0.05in}}
\def \hminb {\hspace{0.15in}}

\def \fgw {1.5in}
\def \fgw {3.6in}
\def \fgh {1.085in}

% \begin{floatingfigure}[r]{2in}  (and \end{..})

\begin{figure}[t!] \centerline{
% \hmina \includegraphics[width=\fgw]{F/empty.eps} \hminb
%\includegraphics[width=\fgw]{F/tmam/eps/membw.pdf} \hminb
        %\includegraphics[width=\fgw]{F/tmam/eps/backend-bound.pdf}
%%%\includegraphics[width=\fgw]{F/tmam/eps/dram+store.pdf}
\hminb
%\includegraphics[width=\fgw]{F/tmam/eps/dram-bound.pdf}
\includegraphics[width=\fgw]{F/tmam/eps/tmam.pdf} }
%
\vminten
%
\mycaption{fig-tmam}{CXL performance slowdown analysis/correlation with
workload and microarchitecture level metrics such as DRAM bandwidth
and DRAM/Store boundness}{}
%
\vminten

\end{figure}



==> tab-cores.tex <==
\newcommand{\ctlen}{.3cm}

%\setlength{\tabcolsep}{4pt}

\begin{table}[t!]
\begin{center}
\small
\centering
%---------------------------------
\begin{tabular}{l|p{\ctlen}p{\ctlen}p{\ctlen}p{\ctlen}p{\ctlen}|r}
& \multicolumn{5}{c|}{Requested CPU Cores per VM}           & {Average} \\
Cluster & 1    & 2    & 4    & 8   & \textgreater{}8 & DRAM/Core \\
\hline
A & 13\% & 11\% & 43\% & 1\% & 32\% & 4 GB     \\
B & 23\% & 24\% & 32\% & 3\% & 18\% & 5.2 GB   \\
C & 16\% & 24\% & 32\% & 2\% & 26\% & 8.8 GB
\end{tabular}
%
%------------ppp---------------------
\end{center}
\vspace{-.1in}
\vminten
%
% Besides different core counts, even within the same datacenter
% (clusters A and C)
\mycaption{tab-cores}{VM Diversity}{Cluster-level diversity of demands
for various types of VMs in terms of CPU cores and DRAM
per core.}
%
\vminten
%
\end{table}



==> tab-findings.tex <==

%\newpage

%\setlength{\tabcolsep}{3pt}

\begin{table*}[th!]
\begin{center}
%\footnotesize
%\small
\begin{tabular}{p{8.5cm}|p{9cm}}
\hline
{\bf Key results, findings and observations} & {\bf Implications / Root causes} \\
\hline
Of the \numTotalApps\ workloads we evaluated, 42\% are not sensitive to CXL latency while some are very sensitive with up to 51\% performance impact. & Even a 90ns latency increase will render full CXL memory backing for VMs impractical, and this validates design decision to keep local DRAM on nodes. \\
\hline
Working set size and DRAM bandwidth are independent of CXL performance while CPI almost perfectly captures it. & We need better methods to predict CXL-caused performace slowdown whereas CPI is a posterior metric. \\
\hline
Peak dram bandwidth for a single workload is less than 40 GB/s. & This validates the design decision that we do not need to interleave across CXL ports. \\
\hline
%Workload specific findings: performance of modern high performance I/O devices (\eg, NVMe SSDs) will be significantly affected; VoltDB is experience much less performance impact than Redis; Spark workload (usually with the highest observable DRAM traffic) are not severely impacted as graph processing workloads. \\
%\hline
\cvn works well if workload footprint fits into the VM's local memory, there will be no performance impact. & We can pool DRAM for \cvn and frigid memory for latency sensitive workloads by only locating frigid memory on pool. \\
\hline
Mixing with 80\% local DRAM ensured good perfornamce for XX-YY\% of workloads -- but tail remains. & A static split between local and CXL DRAM is not sufficient for various types of VMs and workloads. \\
\hline
%Interleaving does not work consistently. \\
\hline
TMA works better than ML and 20\% of workloads can safely be placed entirely into CXL pool & \\
\hline
ML works better than static for frigid memory, and we can safely predict 20\% frigid memory on average, 80\% local memory & \\
\hline
Stranding vs pool size, for different models. & Small pool size is enough and our prediction models make a big difference (\eg, vs. static mixing) \\
\hline
\end{tabular}
\end{center}

\vminfifteen
%
\mycaption{tab-findings}{Summary of evaluation findings}{}
%
%\vminfive

\end{table*}



==> tab-models.tex <==

\setlength{\tabcolsep}{3pt}

\begin{table}[t!]
\begin{center}
%\footnotesize
\small
\begin{tabular}{p{2.8cm}p{2.5cm}p{2.8cm}}
\hline
\textbf{Prediction target}   & \textbf{Purpose}    & \textbf{Inputs (features)} \\
%\hline
Memory footprint             & Allocation decision & Past VM allocations        \\
%\hline
% over future VM lifetime
Lat. sensitivity             & Allocation decision & Past VM allocations        \\
%\hline
% over VM's past lifetime, QoS impact
Lat. sensitivity/QoS & For VM migration    & VM’s runtime history      \\
\hline
\end{tabular}
\end{center}
%
\vminfifteen
%
\mycaption{tbl:predmodels}{Prediction models}{}
%
\vminfifteen
\end{table}


==> tab-rel.tex <==
\newcommand{\rrot}[1]{\begin{rotate}{15} {{#1}} \end{rotate}}
%\renewcommand{\rot}[1]{{\bf {\small #1}}}
%\newcommand{\mycol}[1]{\multicolumn{7}{l}{#1}}
%\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}
%\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcommand{\plen}{.8cm}

\setlength{\tabcolsep}{5pt}

\begin{table}[t!]
\begin{center}
\small
\centering
\vspace*{12pt}
%---------------------------------
% p{5.5cm}
\hspace*{-10pt}
\begin{tabular}{l|p{\plen}p{\plen}p{\plen}p{\plen}p{\plen}}
%{\bf Requirements} \
& \rrot{{HW} \cite{thymesisflow.micro20,zombieland.eurosys18, pberry.hotos19, dredbox.date16, memblade.isca09, optmemdisagg, mind.corr21}} \
%& \rrot{ZRAM \cite{softfarmem.asplos19}} \
& \rrot{{VMM/OS} \cite{infiniswap.nsdi17, legoos.osdi18, softfarmem.asplos19, dcm.tc19, fastswap.eurosys20, leap.atc20, fluidmem.icdcs20, orchdisaggmem.tc20, ememdisagg.corr20}} \
& \rrot{{Runtime} \cite{aifm.osdi20, semeru.osdi20, kona.asplos21}} \
& \rrot{{App} \cite{farm.nsdi14, remoteregions.atc18, kvdisagg.atc20, farview.corr21}} \
& \rrot{\bf \sys} \\
\hline
%&  & \cite{flash.isca94} & \cite{softfarmem.asplos19} & \cite{infiniswap.nsdi17,fastswap.eurosys20} & \cite{leap.atc20} & \cite{aifm.osdi20, semeru.osdi20, kona.asplos21} & \cite{thymesisflow.micro20} \\
%\hline
%{App Transparency} & \xm       & \xm     & \xm      & \xm      & \cm             \\
{Inertia}      		& \cm       & \cm     & \cm      & \xm      & \cm            \\
%{For-VM-use}       & \cm       & \xm     & \xm      & \xm      & \cm            \\
%\rowcolor{Gray!30}
{Performance}       & \cm       & \xm      & \xm      & \xm      & \cm            \\
%{VM/DDA}           & \cm       & \xm     & \xm      & \xm      & \cm            \\
{Deployability}     & \xm       & \cm     & \cm      & \cm      & \cm            \\
%\rowcolor{Gray!30}
{VirtAccel} 		& \cm       & \xm     & \cm      & \cm      & \cm            \\
{CpuEfficiency}     & \cm       & \xm     & \xm      & \xm      & \cm            \\
%{Interconnect}     & \ts{CAPI} & --      & \ts{Net} & \ts{Net} & \ts{CXL}   \\
%{Pool size}        & \ts{Rack} & \ts{DC} & \ts{DC}  & \ts{DC}  & \ts{Rack}   \\
%{Deployable}       & \xm       & \cm     & \cm      & \xm      & \cm            \\
%\hline
\end{tabular}
%------------ppp---------------------
\end{center}

\vminten
%
\mycaption{tab-rel}{\sys vs. state-of-the-art
    memory disaggregation approaches (\sec\ref{sec-rel})}{\sys satisfies many key requirements
and is practical for cloud datacenters.}
% deployment, transparent to VMs/applications, and achieves comparable
% performance to today's clouds.
%
% \hcl{TODO: ``Scope'' row, ``Deployment'' \ra Commodity CPU}
%
%\vspace*{-12pt}
\vminfifteen

\end{table}


